GBSVR: Granular Ball Support Vector Regression

Support Vector Regression (SVR) and its variants are widely used to handle regression tasks, however, since their solution involves solving an expensive quadratic programming problem, it limits its application, especially when dealing with large datasets. Additionally, SVR uses an epsilon-insensitive loss function which is sensitive to outliers and therefore can adversely affect its performance. We propose Granular Ball Support Vector Regression (GBSVR) to tackle problem of regression by using granular ball concept. These balls are useful in simplifying complex data spaces for machine learning tasks, however, to the best of our knowledge, they have not been sufficiently explored for regression problems. Granular balls group the data points into balls based on their proximity and reduce the computational cost in SVR by replacing the large number of data points with far fewer granular balls. This work also suggests a discretization method for continuous-valued attributes to facilitate the construction of granular balls. The effectiveness of the proposed approach is evaluated on several benchmark datasets and it outperforms existing state-of-the-art approaches

==> Ablation_min_pts.tex <==
% Images for Time Series
\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/R2_vs_min_points.png} % Path to your first image
        \centering % Center the text
        \text{$R^2$}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/MAE_vs_min_points.png} % Path to your second image
        \centering % Center the text
        \text{MAE}
    \end{minipage}

    \vspace{1em}

    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/MSE_vs_min_points.png} % Path to your third image
        \centering % Center the text
        \text{MSE}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/RMSE_vs_min_points.png} % Path to your fourth image
        \centering % Center the text
        \text{RMSE}
    \end{minipage}
    
    \vspace{1em}
    \centering
    \caption{Ablation Studies on Minimum Number of points in each Ball} % This text is already centered
    \label{ablation_minPts}
\end{figure*}

==> Artificial_Data/cos_table.tex <==

\begin{table}[ht]
\scriptsize
\centering
\caption{Comparison results of three models with six different types of noise on Type B dataset.}
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l|cccc|cccc|}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{Type 1 Noise}} & \multicolumn{4}{c|}{\textbf{Type 2 Noise}} \\
\cline{2-9}
& \textbf{R$^2$} & \textbf{MAE} & \textbf{MSE} & \textbf{RMSE} & \textbf{R$^2$} & \textbf{MAE} & \textbf{MSE} & \textbf{RMSE} \\
\hline
GBSVR & \textbf{0.9919} & \textbf{0.0523} & \textbf{0.0041} & \textbf{0.0641} & \textbf{0.9920} & \textbf{0.0527} & \textbf{0.0039} & \textbf{0.0624} \\
SVR   & 0.9867 & 0.0682 & 0.0067 & 0.0816 & 0.9868 & 0.0651 & 0.0065 & 0.0805 \\
NuSVR & 0.9653 & 0.1181 & 0.0183 & 0.1353 & 0.9756 & 0.0946 & 0.0127 & 0.1125 \\
\hline
\end{tabular}
\vspace{0.5cm}

\begin{tabular}{|l|cccc|cccc|}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{Type 3 Noise}} & \multicolumn{4}{c|}{\textbf{Type 4 Noise}} \\
\cline{2-9}
& \textbf{R$^2$} & \textbf{MAE} & \textbf{MSE} & \textbf{RMSE} & \textbf{R$^2$} & \textbf{MAE} & \textbf{MSE} & \textbf{RMSE} \\
\hline
GBSVR & \textbf{0.9998} & \textbf{0.0085} & \textbf{0.0001} & \textbf{0.0103} & \textbf{0.9999} & 0.0059 & 0.0001 & 0.0072 \\
SVR   & 0.9996 & 0.0112 & 0.0002 & 0.0133 & 0.9999 & \textbf{0.0052} & \textbf{0.0000} & \textbf{0.0066} \\
NuSVR & 0.9996 & 0.0114 & 0.0002 & 0.0137 & 0.9999 & 0.0058 & 0.0001 & 0.0071 \\
\hline
\end{tabular}
\vspace{0.5cm}

\begin{tabular}{|l|cccc|cccc|}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{Type 5 Noise}} & \multicolumn{4}{c|}{\textbf{Type 6 Noise}} \\
\cline{2-9}
& \textbf{R$^2$} & \textbf{MAE} & \textbf{MSE} & \textbf{RMSE} & \textbf{R$^2$} & \textbf{MAE} & \textbf{MSE} & \textbf{RMSE} \\
\hline
GBSVR & \textbf{0.9945} & \textbf{0.0429} & \textbf{0.0028} & \textbf{0.0525} & \textbf{0.9939} & \textbf{0.0444} & \textbf{0.0029} & \textbf{0.0535} \\
SVR   & 0.9916 & 0.0541 & 0.0043 & 0.0657 & 0.9918 & 0.0516 & 0.0041 & 0.0644 \\
NuSVR & 0.9779 & 0.0912 & 0.0107 & 0.1035 & 0.9812 & 0.0799 & 0.0091 & 0.0952 \\
\hline
\end{tabular}
\label{cos_table}
\end{table}

==> ablation_purity.tex <==
% Images for Time Series
\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/R2_vs_purity.png} % Path to your first image
        \centering % Center the text
        \text{$R^2$}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/MAE_vs_purity.png} % Path to your second image
        \centering % Center the text
        \text{MAE}
    \end{minipage}

    \vspace{1em}

    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/MSE_vs_purity.png} % Path to your third image
        \centering % Center the text
        \text{MSE}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/RMSE_vs_purity.png} % Path to your fourth image
        \centering % Center the text
        \text{RMSE}
    \end{minipage}
    
    \vspace{1em}
    \centering
    \caption{Ablation Studies on Purity} % This text is already centered
    \label{abalation_purity}
    \label{ablation_purity}
\end{figure*}

% Images for Time Series
\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/R2_vs_min_points.png} % Path to your first image
        \centering % Center the text
        \text{$R^2$}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/MAE_vs_min_points.png} % Path to your second image
        \centering % Center the text
        \text{MAE}
    \end{minipage}

    \vspace{1em}

    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/MSE_vs_min_points.png} % Path to your third image
        \centering % Center the text
        \text{MSE}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Ablation/RMSE_vs_min_points.png} % Path to your fourth image
        \centering % Center the text
        \text{RMSE}
    \end{minipage}
    
    \vspace{1em}
    \centering
    \caption{Ablation Studies on Minimum Number of points in each Ball} % This text is already centered
    \label{ablation_minPts}
\end{figure*}

==> conMGSVR/con.tex <==
% Images for Time Series
\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{conMGSVR/outputs.png} % Path to your first image
        \centering % Center the caption
        \text{$-cos(x) exp( -(x - \pi )^2 )$}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{conMGSVR/con_cos.png} % Path to your second image
        \centering % Center the caption
        \text{$cos(\pi x)$}
    \end{minipage}

    \vspace{1em}

    
    
    \vspace{1em}
    \centering
    \caption{ConMGSVR vs GBSVR} % This caption is already centered
    \label{conMGSVR}
\end{figure*}

==> graphs/Ballgeneration.tex <==
% \begin{figure*}[ht]
%     \centering
    
%     % First row
%     \begin{minipage}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{graphs/Ball Generation/0.png}
%         \text{Step 1}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{graphs/Ball Generation/1.png}
%         \text{Step 2}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{graphs/Ball Generation/2.png}
%         \text{Step 3}
%     \end{minipage}

%     \vskip 0.5cm

%     % Second row
%     \begin{minipage}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{graphs/Ball Generation/3.png}
%         \text{Step 4}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{graphs/Ball Generation/4.png}
%         \text{Step 5}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{graphs/Ball Generation/5.png}
%         \text{Step 6}
%     \end{minipage}

%     \caption{Granular Regression Ball  Generation Process}
%     \label{fig:Steps_grid}
% \end{figure*}

\begin{figure*}[ht]
    \centering
    % First row
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/Ball Generation/0.png}
        \text{Step 1}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/Ball Generation/1.png}
        \text{Step 2}
    \end{minipage}

    \vskip 0.5cm

    % Second row
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/Ball Generation/2.png}
        \text{Step 3}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/Ball Generation/3.png}
        \text{Step 4}
    \end{minipage}

    \vskip 0.5cm

    % Third row
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/Ball Generation/4.png}
        \text{Step 5}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/Ball Generation/5.png}
        \text{Step 6}
    \end{minipage}

    \caption{Granular Regression Ball Generation Process}
    \label{fig:Steps_grid}
\end{figure*}


==> graphs/cos_all.tex <==
% Two Rows of Images (3 in each row)
\begin{figure*}[ht]
    \centering
    % First row with 3 images
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_1.png} % Path to your first image
        \text{Type 1}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_2.png} % Path to your second image
        \text{Type 2}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_3.png} % Path to your third image
        \text{Type 3}
    \end{minipage}
    
    \vspace{1em}

    % Second row with 3 images
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_4.png} % Path to your fourth image
        \text{Type 4}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_5.png} % Path to your fifth image
        \text{Type 5}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_6.png} % Path to your sixth image
        \text{Type 6}
    \end{minipage}
    
    \vspace{1em}
    \centering
    \caption{Type B dataset}
    \label{cos_graphs}
\end{figure*}


==> graphs/sinc_all.tex <==

\begin{figure*}[ht]
    \centering
    % First row with 3 images
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/sinc/Type_1.png} % Path to your first image
        \text{Type 1}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/sinc/Type_2.png} % Path to your second image
        \text{Type 2}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/sinc/Type_3.png} % Path to your third image
        \text{Type 3}
    \end{minipage}
    
    \vspace{1em}

    % Second row with 3 images
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/sinc/Type_4.png} % Path to your fourth image
        \text{Type 4}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/sinc/Type_5.png} % Path to your fifth image
        \text{Type 5}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/sinc/Type_6.png} % Path to your sixth image
        \text{Type 6}
    \end{minipage}
    
    \vspace{1em}
    \centering
    \caption{Type A dataset}
    \label{sinc_graphs}
\end{figure*}

% Two Rows of Images (3 in each row)
\begin{figure*}[ht]
    \centering
    % First row with 3 images
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_1.png} % Path to your first image
        \text{Type 1}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_2.png} % Path to your second image
        \text{Type 2}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_3.png} % Path to your third image
        \text{Type 3}
    \end{minipage}
    
    \vspace{1em}

    % Second row with 3 images
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_4.png} % Path to your fourth image
        \text{Type 4}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_5.png} % Path to your fifth image
        \text{Type 5}
    \end{minipage}
    \hfill
    \begin{minipage}{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/cosx/Type_6.png} % Path to your sixth image
        \text{Type 6}
    \end{minipage}
    
    \vspace{1em}
    \centering
    \caption{Type B dataset}
    \label{cos_graphs}
\end{figure*}


==> graphs/timeseries_all.tex <==
% Images for Time Series
\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/stocks/AAPL_zoom.png} % Path to your first image
        \centering % Center the caption
        \text{APPLE}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/stocks/GOOGL.png} % Path to your second image
        \centering % Center the text
        \text{GOOGLE}
    \end{minipage}

    \vspace{1em}

    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/stocks/NVDA.png} % Path to your third image
        \centering % Center the text
        \text{NVIDIA}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/stocks/TSLA.png} % Path to your fourth image
        \centering % Center the text
        \text{TESLA}
    \end{minipage}
    
    \vspace{1em}
    \centering
    \caption{Stock price forecasting} % This caption is already centered
    \label{stock_price}
\end{figure*}


% Images for wind Data
\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/wind/20_min.png} % Path to your first image
        \centering % Center the caption
        \text{20 min interval}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/wind/30_min.png} % Path to your second image
        \centering % Center the caption
        \text{30 min interval}
    \end{minipage}

    \centering % Center the caption
     \caption{Wind Speed Prediction}
      \label{wind_speed_graphs}
\end{figure*}

==> graphs/wind_all.tex <==
% Images for wind Data
\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/wind/20_min.png} % Path to your first image
        \centering % Center the caption
        \text{20 min interval}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{graphs/wind/30_min.png} % Path to your second image
        \centering % Center the caption
        \text{30 min interval}
    \end{minipage}

    \centering % Center the caption
     \caption{Wind Speed Prediction}
      \label{wind_speed_graphs}
\end{figure*}

==> result_table2.tex <==


% \include{tables}

% % \cellcolor{gray!35}\textbf{Yeast} \\
% % \cellcolor{gray!35}\textbf{emotions} \\
% % \cellcolor{gray!35}\textbf{Scene}   \\
% % \cellcolor{gray!35}\textbf{image}   \\
% \include{graphLap}

% \setlength{\arrayrulewidth}{2pt}
\begin{table*}[]
\normalsize
\centering
\caption{COMPARISON OF PERFORMANCE BETWEEN DIFFERENT METHODS WITH DIFFERENT LEVELS OF NOISE }
\begin{tabular}{|l|l|c|c|c|c|c|c|}
\hline

\multicolumn{7}{|c|}{autos} \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
\textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \hline
\multirow{3}{*}{\textbf{Time $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{1.11±0.112}     & \textbf{1.113±0.152}     & \textbf{1.111±0.115}    & \textbf{1.11±0.174}     & \textbf{1.227±0.139}   \\ \hline
              & \textbf{SVR}       & 9.416±0.371    & 9.389±0.285     & 9.124±0.354    & 9.468±0.568    & 9.576±0.456    \\ \hline
              & \textbf{Nu-SVR}    & 8.464±0.559    & 8.401±0.45      & 8.276±0.765    & 8.438±0.589    & 8.564±0.549    \\ \Xhline{3\arrayrulewidth}


\multirow{3}{*}{\textbf{$R^2$ $(\uparrow)$ }} 
              & \textbf{GBSVR}     & \textbf{0.872±0.037}    & \textbf{0.873±0.039}     & \textbf{0.872±0.025}    & \textbf{0.89±0.024}     & \textbf{0.875±0.028}    \\ \hline
              & \textbf{SVR}       & 0.74±0.068     & 0.725±0.093     & 0.701±0.087    & 0.789±0.068    & 0.715±0.137    \\ \hline
              & \textbf{Nu-SVR}    & 0.839±0.035    & 0.845±0.033     & 0.829±0.047    & 0.824±0.05     & 0.835±0.052    \\ \Xhline{3\arrayrulewidth}
              
\multirow{3}{*}{\textbf{MAE $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.265±0.032}    & \textbf{0.264±0.017}     & \textbf{0.266±0.034}    & \textbf{0.253±0.026}    & \textbf{0.262±0.021}    \\ \hline
              & \textbf{SVR}       & 0.356±0.033    & 0.353±0.033     & 0.367±0.035    & 0.322±0.034    & 0.355±0.056    \\ \hline
              & \textbf{Nu-SVR}    & 0.285±0.039    & 0.286±0.046     & 0.292±0.042    & 0.301±0.041    & 0.284±0.046    \\ \Xhline{3\arrayrulewidth}

\multirow{3}{*}{\textbf{MSE $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.119±0.022}    & \textbf{0.116±0.015}     & \textbf{0.121±0.024}    & \textbf{0.104±0.02}    & \textbf{0.116±0.014}    \\ \hline
              & \textbf{SVR}       & 0.249±0.071    & 0.256±0.078     & 0.275±0.06     & 0.192±0.032    & 0.26±0.106     \\ \hline
              & \textbf{Nu-SVR}    & 0.157±0.051    & 0.152±0.054     & 0.161±0.044    & 0.167±0.051    & 0.163±0.074    \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{RMSE $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.344±0.032}    & \textbf{0.339±0.023}     & \textbf{0.347±0.036}    & \textbf{0.321±0.031}    & \textbf{0.341±0.021}    \\ \hline
              & \textbf{SVR}       & 0.493±0.076    & 0.5±0.079       & 0.521±0.059    & 0.436±0.037    & 0.499±0.103    \\ \hline
              & \textbf{Nu-SVR}    & 0.391±0.065    & 0.384±0.068     & 0.397±0.056    & 0.404±0.064    & 0.394±0.086    \\ \Xhline{3\arrayrulewidth}





\multicolumn{7}{|c|}{machine} \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
\textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \hline
\multirow{3}{*}{\textbf{Time($\downarrow$)}} 
              & \textbf{GBSVR}  & \textbf{1.888±0.115}     & \textbf{1.902±0.136}     & \textbf{1.918±0.126}     & \textbf{1.993±0.177}    & \textbf{2.069±0.153}    \\ \hline
              & \textbf{SVR}    & 17.078±0.233    & 16.954±0.226    & 16.993±0.262    & 17.053±0.229   & 16.952±0.251   \\ \hline
              & \textbf{Nu-SVR} & 17.222±0.269    & 17.12±0.297     & 17.165±0.261    & 17.2±0.248     & 17.13±0.301    \\ 

\Xhline{3\arrayrulewidth}  


              
\multirow{3}{*}{\textbf{$R^2$($\uparrow$)}} 
              & \textbf{GBSVR}  & \textbf{0.836±0.021}     & \textbf{0.834±0.027}     & \textbf{0.835±0.032}     & \textbf{0.82±0.042}    & \textbf{0.826±0.036}    \\ \hline
              & \textbf{SVR}    & 0.744±0.065     & 0.743±0.053     & 0.718±0.103     & 0.734±0.057   & 0.746±0.046   \\ \hline
              & \textbf{Nu-SVR} & 0.746±0.035     & 0.748±0.036     & 0.753±0.037     & 0.749±0.036   & 0.747±0.034   \\ 

\Xhline{3\arrayrulewidth} 
              
\multirow{3}{*}{\textbf{MAE  $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.311±0.023}     & \textbf{0.311±0.03}     & \textbf{0.308±0.023}     & \textbf{0.321±0.023}    & \textbf{0.32±0.021}    \\ \hline
              & \textbf{SVR}    & 0.376±0.071     & 0.384±0.068    & 0.388±0.078     & 0.385±0.069   & 0.379±0.062   \\ \hline
              & \textbf{Nu-SVR} & 0.392±0.033     & 0.392±0.033    & 0.39±0.037      & 0.392±0.036   & 0.389±0.036   \\ 

\Xhline{3\arrayrulewidth}


\multirow{3}{*}{\textbf{MSE  $(\downarrow)$}} 
               & \textbf{GBSVR}  & \textbf{0.161±0.026}     & \textbf{0.161±0.025}     & \textbf{0.16±0.027}     & \textbf{0.173±0.022}    & \textbf{0.168±0.026}    \\ \hline
              & \textbf{SVR}    & 0.258±0.104     & 0.257±0.088    & 0.288±0.155     & 0.267±0.094   & 0.252±0.074   \\ \hline
              & \textbf{Nu-SVR} & 0.247±0.031     & 0.245±0.029    & 0.241±0.036     & 0.244±0.033   & 0.247±0.034   \\ 

\Xhline{3\arrayrulewidth} 


\multirow{3}{*}{\textbf{RMSE  $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.4±0.033}       & \textbf{0.401±0.031}     & \textbf{0.399±0.033}     & \textbf{0.414±0.027}    & \textbf{0.409±0.031}    \\ \hline
              & \textbf{SVR}    & 0.499±0.091     & 0.501±0.079     & 0.522±0.126     & 0.51±0.082     & 0.498±0.067    \\ \hline
              & \textbf{Nu-SVR} & 0.496±0.031     & 0.494±0.03      & 0.489±0.036     & 0.493±0.033    & 0.495±0.033    \\ 

\Xhline{3\arrayrulewidth}  



\multicolumn{7}{|c|}{Real Estate Valuation} \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
\textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \hline
\multirow{3}{*}{\textbf{Time $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{7.335±1.151}     & \textbf{7.121±0.633}     & \textbf{6.86±0.881}      & \textbf{8.004±1.186}    & \textbf{7.522±0.642}    \\ \hline
              & \textbf{SVR}    & 95.774±0.917    & 94.793±0.865    & 94.927±0.703    & 96.663±1.722   & 95.103±0.671   \\ \hline
              & \textbf{Nu-SVR} & 93.068±1.192    & 92.017±1.501    & 91.805±0.768    & 94.193±1.282   & 91.832±0.746   \\ 

\Xhline{3\arrayrulewidth}  


              
\multirow{3}{*}{\textbf{$R^2$ $(\uparrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.63±0.075 }     & \textbf{0.629±0.069}     & \textbf{0.633±0.077}     & \textbf{0.637±0.073}    & \textbf{0.625±0.071}    \\ \hline
              & \textbf{SVR}    & 0.542±0.059     & 0.546±0.07      & 0.535±0.062     & 0.555±0.066    & 0.531±0.057    \\ \hline
              & \textbf{Nu-SVR} & 0.548±0.061     & 0.557±0.071     & 0.54±0.065      & 0.553±0.059    & 0.53±0.06      \\ 

\Xhline{3\arrayrulewidth}  


              
\multirow{3}{*}{\textbf{MAE $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.403±0.034}     & \textbf{0.4±0.032}       & \textbf{0.4±0.033}       & \textbf{0.395±0.032}    & \textbf{0.403±0.03}     \\ \hline
              & \textbf{SVR}    & 0.503±0.035     & 0.5±0.037       & 0.507±0.035     & 0.499±0.039    & 0.508±0.03     \\ \hline
              & \textbf{Nu-SVR} & 0.5±0.034       & 0.495±0.04      & 0.504±0.038     & 0.498±0.03     & 0.511±0.036    \\ 

\Xhline{3\arrayrulewidth}  



\multirow{3}{*}{\textbf{MSE $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.374±0.132}     & \textbf{0.375±0.126}     & \textbf{0.372±0.134}     & \textbf{0.367±0.127}    & \textbf{0.379±0.128}    \\ \hline
              & \textbf{SVR}    & 0.455±0.098     & 0.45±0.1        & 0.463±0.105     & 0.443±0.105    & 0.466±0.104    \\ \hline
              & \textbf{Nu-SVR} & 0.448±0.098     & 0.439±0.103     & 0.458±0.107     & 0.444±0.096    & 0.467±0.101    \\ 

\Xhline{3\arrayrulewidth} 


\multirow{3}{*}{\textbf{RMSE  $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.604±0.099}     & \textbf{0.605±0.094}     & \textbf{0.601±0.1}       & \textbf{0.598±0.096}    & \textbf{0.608±0.096}    \\ \hline
              & \textbf{SVR}    & 0.671±0.069     & 0.667±0.071     & 0.676±0.073     & 0.661±0.075    & 0.679±0.072    \\ \hline
              & \textbf{Nu-SVR} & 0.666±0.069     & 0.659±0.075     & 0.672±0.075     & 0.663±0.069    & 0.68±0.07      \\ 

\Xhline{3\arrayrulewidth}  





\end{tabular}
\label{result_table2}
\end{table*}




==> result_table_uci.tex <==


% \include{tables}

% % \cellcolor{gray!35}\textbf{Yeast} \\
% % \cellcolor{gray!35}\textbf{emotions} \\
% % \cellcolor{gray!35}\textbf{Scene}   \\
% % \cellcolor{gray!35}\textbf{image}   \\
% \include{graphLap}

% \setlength{\arrayrulewidth}{2pt}
\begin{table*}[]
\tiny
\centering
\caption{COMPARISON OF PERFORMANCE BETWEEN DIFFERENT METHODS WITH DIFFERENT LEVELS OF NOISE }

\begin{tabular}{|l|l|c|c|c|c|c|c|}
\hline

\multicolumn{7}{|c|}{servo} \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
\textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{Time  $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.996±0.058}    & \textbf{1.039±0.069}     & \textbf{1.023±0.063}    & \textbf{1.088±0.08}     & \textbf{1.082±0.049}    \\ \hline
              & \textbf{SVR}       & 9.289±0.116    & 9.3±0.098       & 9.319±0.124    & 9.374±0.097    & 9.351±0.095    \\ \hline
              & \textbf{Nu-SVR}    & 4.729±0.104    & 4.902±0.231     & 4.903±0.23     & 4.889±0.291    & 4.612±0.281    \\ \Xhline{3\arrayrulewidth}

\multirow{3}{*}{\textbf{$R^2$  $(\uparrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.855±0.014}    & \textbf{0.856±0.032}    & \textbf{0.863±0.031}    & \textbf{0.834±0.032}    & \textbf{0.846±0.039}    \\ \hline
              & \textbf{SVR}       & 0.773±0.08     & 0.707±0.124    & 0.739±0.115    & 0.612±0.199    & 0.756±0.048    \\ \hline
              & \textbf{Nu-SVR}    & 0.836±0.03     & 0.833±0.03     & 0.817±0.052    & 0.811±0.041    & 0.833±0.044    \\ \Xhline{3\arrayrulewidth}
              
\multirow{3}{*}{\textbf{MAE  $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.274±0.009}    & \textbf{0.262±0.024}    & \textbf{0.256±0.038}    & \textbf{0.286±0.023}    & \textbf{0.276±0.036}    \\ \hline
              & \textbf{SVR}       & 0.366±0.063    & 0.424±0.104    & 0.384±0.047    & 0.473±0.124    & 0.394±0.077    \\ \hline
              & \textbf{Nu-SVR}    & 0.298±0.019    & 0.301±0.028    & 0.325±0.049    & 0.323±0.021    & 0.305±0.033    \\ \Xhline{3\arrayrulewidth}
              
\multirow{3}{*}{\textbf{MSE  $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.142±0.022}    & \textbf{0.138±0.024}    & \textbf{0.137±0.048}    & \textbf{0.161±0.031}    & \textbf{0.152±0.047}    \\ \hline
              & \textbf{SVR}       & 0.217±0.073    & 0.289±0.135    & 0.241±0.067    & 0.377±0.180    & 0.243±0.072    \\ \hline
              & \textbf{Nu-SVR}    & 0.159±0.032    & 0.163±0.035    & 0.179±0.058    & 0.182±0.032    & 0.164±0.051    \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{RMSE $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.376±0.029}    & \textbf{0.370±0.032}    & \textbf{0.365±0.062}    & \textbf{0.399±0.040}    & \textbf{0.385±0.062}    \\ \hline
              & \textbf{SVR}       & 0.459±0.077    & 0.524±0.120    & 0.487±0.067    & 0.599±0.136    & 0.488±0.073    \\ \hline
              & \textbf{Nu-SVR}    & 0.397±0.038    & 0.402±0.042    & 0.418±0.067    & 0.425±0.036    & 0.400±0.059    \\ \Xhline{3\arrayrulewidth}



\multicolumn{7}{|c|}{Yacth} \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
\textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{Time($\downarrow$)}} 
              & \textbf{GBSVR}  & \textbf{1.194±0.29}     & \textbf{1.076±0.274}                       & \textbf{1.003±0.27}     & \textbf{1.102±0.334}    & \textbf{1.187±0.283}    \\ \hline
              & \textbf{SVR}    & 41.285±0.356   & 41.118±0.441                      & 40.199±0.453   & 42.357±1.694   & 41.433±0.395   \\ \hline
              & \textbf{Nu-SVR} & 37.262±0.179   & 37.798±0.23                       & 37.588±0.425   & 40.393±1.299   & 37.534±0.235   \\ 
          
               \Xhline{3\arrayrulewidth}

\multirow{3}{*}{\textbf{$R^2$$ (\uparrow) $}} 
              & \textbf{GBSVR}     & \textbf{0.968±0.014}    & \textbf{0.969±0.015}     & \textbf{0.968±0.015}    & \textbf{0.966±0.015}    & \textbf{0.968±0.014}    \\ \hline
              & \textbf{SVR}       & 0.962±0.021    & 0.966±0.017     & 0.952±0.016    & 0.960±0.008    & 0.962±0.021    \\ \hline
              & \textbf{Nu-SVR}    & 0.966±0.016    & 0.964±0.015     & 0.963±0.017    & 0.964±0.015    & 0.966±0.016    \\ \Xhline{3\arrayrulewidth}

\multirow{3}{*}{\textbf{MAE $ (\downarrow) $}} 
              & \textbf{GBSVR}     & \textbf{0.105±0.021}    & \textbf{0.104±0.019}     & \textbf{0.106±0.018}    & \textbf{0.111±0.02}     & \textbf{0.105±0.021}    \\ \hline
              & \textbf{SVR}       & 0.13±0.031     & 0.122±0.023     & 0.16±0.035     & 0.143±0.009    & 0.13±0.031     \\ \hline
              & \textbf{Nu-SVR}    & 0.105±0.02     & 0.107±0.016     & 0.111±0.015    & 0.112±0.015    & 0.105±0.02     \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{MSE $ (\downarrow) $}} 
              & \textbf{GBSVR}     & \textbf{0.032±0.019}    & \textbf{0.031±0.02}      & \textbf{0.032±0.02}     & \textbf{0.034±0.02}    & \textbf{0.032±0.019}    \\ \hline
              & \textbf{SVR}       & 0.039±0.029    & 0.034±0.022     & 0.049±0.022    & 0.041±0.014    & 0.039±0.029    \\ \hline
              & \textbf{Nu-SVR}    & 0.035±0.021    & 0.037±0.02      & 0.037±0.021    & 0.036±0.019    & 0.035±0.021    \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{RMSE($\downarrow$)}} 
              & \textbf{GBSVR}     & \textbf{0.173±0.051}    & \textbf{0.17±0.051}      & \textbf{0.172±0.052}    & \textbf{0.178±0.05}     & \textbf{0.173±0.051}    \\ \hline
              & \textbf{SVR}       & 0.187±0.064    & 0.176±0.054     & 0.214±0.051    & 0.199±0.033    & 0.187±0.064    \\ \hline
              & \textbf{Nu-SVR}    & 0.179±0.052    & 0.185±0.049     & 0.186±0.052    & 0.184±0.046    & 0.179±0.052    \\ \Xhline{3\arrayrulewidth}


\multicolumn{7}{|c|}{autompg} \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
\textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \hline
\multirow{3}{*}{\textbf{Time($\downarrow$)}} 
              & \textbf{GBSVR}     & \textbf{7.234±0.524}    & \textbf{6.813±0.502}     & \textbf{7.46±0.511}     & \textbf{7.664±0.587}    & \textbf{7.029±0.556}    \\ \hline
              & \textbf{SVR}       & 69.362±0.425   & 69.68±0.464     & 70.256±0.515   & 70.323±0.466   & 71.437±0.469   \\ \hline
              & \textbf{Nu-SVR}    & 85.806±0.699   & 85.985±0.661    & 45.173±4.906   & 34.241±2.73    & 31.724±3.354   \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{$R^2$  $(\uparrow)$}}               & \textbf{GBSVR}     & \textbf{0.866±0.016}    & \textbf{0.848±0.019}     & \textbf{0.864±0.012}    & \textbf{0.846±0.028}    & \textbf{0.84±0.023}     \\ \hline
              & \textbf{SVR}       & 0.787±0.056    & 0.777±0.037     & 0.663±0.297    & 0.754±0.05     & 0.753±0.058    \\ \hline
              & \textbf{Nu-SVR}    & 0.812±0.028    & 0.81±0.028      & 0.817±0.033    & 0.817±0.031    & 0.802±0.034    \\ \Xhline{3\arrayrulewidth}
              
\multirow{3}{*}{\textbf{MAE  $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.27±0.028}     & \textbf{0.276±0.021}     & \textbf{0.268±0.022}    & \textbf{0.283±0.046}    & \textbf{0.298±0.035}    \\ \hline
              & \textbf{SVR}       & 0.364±0.068    & 0.367±0.018     & 0.428±0.187    & 0.366±0.038    & 0.379±0.052    \\ \hline
              & \textbf{Nu-SVR}    & 0.347±0.029    & 0.35±0.028      & 0.311±0.03     & 0.309±0.047    & 0.311±0.033    \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{MSE  $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.133±0.028}    & \textbf{0.15±0.021}      & \textbf{0.133±0.01}7    & \textbf{0.154±0.038}    & \textbf{0.16±0.038}     \\ \hline
              & \textbf{SVR}       & 0.214±0.077    & 0.216±0.022     & 0.327±0.282    & 0.24±0.041     & 0.243±0.058    \\ \hline
              & \textbf{Nu-SVR}    & 0.186±0.036    & 0.188±0.035     & 0.182±0.045    & 0.185±0.057    & 0.198±0.054    \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{RMSE  $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.363±0.039}    & \textbf{0.386±0.028}     & \textbf{0.365±0.023}    & \textbf{0.389±0.04}9    & \textbf{0.397±0.049}    \\ \hline
              & \textbf{SVR}       & 0.455±0.082    & 0.464±0.024     & 0.533±0.207    & 0.488±0.041    & 0.489±0.057    \\ \hline
              & \textbf{Nu-SVR}    & 0.429±0.041    & 0.432±0.04      & 0.424±0.054    & 0.425±0.063    & 0.441±0.061    \\ \Xhline{3\arrayrulewidth}



% \multicolumn{7}{|c|}{autos} \\ \Xhline{3\arrayrulewidth}
% \multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
% \textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \hline
% \multirow{3}{*}{\textbf{Time}} 
%               & \textbf{GBSVR}     & 1.11±0.112     & 1.113±0.152     & 1.111±0.115    & 1.11±0.174     & 1.227±0.139    \\ \hline
%               & \textbf{SVR}       & 9.416±0.371    & 9.389±0.285     & 9.124±0.354    & 9.468±0.568    & 9.576±0.456    \\ \hline
%               & \textbf{Nu-SVR}    & 8.464±0.559    & 8.401±0.45      & 8.276±0.765    & 8.438±0.589    & 8.564±0.549    \\ \Xhline{3\arrayrulewidth}
              
% \multirow{3}{*}{\textbf{$R^2$}} 
%               & \textbf{GBSVR}     & 0.872±0.037    & 0.873±0.039     & 0.872±0.025    & 0.89±0.024     & 0.875±0.028    \\ \hline
%               & \textbf{SVR}       & 0.74±0.068     & 0.725±0.093     & 0.701±0.087    & 0.789±0.068    & 0.715±0.137    \\ \hline
%               & \textbf{Nu-SVR}    & 0.839±0.035    & 0.845±0.033     & 0.829±0.047    & 0.824±0.05     & 0.835±0.052    \\ \Xhline{3\arrayrulewidth}
              
% \multirow{3}{*}{\textbf{MAE}} 
%               & \textbf{GBSVR}     & 0.265±0.032    & 0.264±0.017     & 0.266±0.034    & 0.253±0.026    & 0.262±0.021    \\ \hline
%               & \textbf{SVR}       & 0.356±0.033    & 0.353±0.033     & 0.367±0.035    & 0.322±0.034    & 0.355±0.056    \\ \hline
%               & \textbf{Nu-SVR}    & 0.285±0.039    & 0.286±0.046     & 0.292±0.042    & 0.301±0.041    & 0.284±0.046    \\ \Xhline{3\arrayrulewidth}

% \multirow{3}{*}{\textbf{MSE}} 
%               & \textbf{GBSVR}     & 0.119±0.022    & 0.116±0.015     & 0.121±0.024    & 0.104±0.02     & 0.116±0.014    \\ \hline
%               & \textbf{SVR}       & 0.249±0.071    & 0.256±0.078     & 0.275±0.06     & 0.192±0.032    & 0.26±0.106     \\ \hline
%               & \textbf{Nu-SVR}    & 0.157±0.051    & 0.152±0.054     & 0.161±0.044    & 0.167±0.051    & 0.163±0.074    \\ \Xhline{3\arrayrulewidth}
% \multirow{3}{*}{\textbf{RMSE}} 
%               & \textbf{GBSVR}     & 0.344±0.032    & 0.339±0.023     & 0.347±0.036    & 0.321±0.031    & 0.341±0.021    \\ \hline
%               & \textbf{SVR}       & 0.493±0.076    & 0.5±0.079       & 0.521±0.059    & 0.436±0.037    & 0.499±0.103    \\ \hline
%               & \textbf{Nu-SVR}    & 0.391±0.065    & 0.384±0.068     & 0.397±0.056    & 0.404±0.064    & 0.394±0.086    \\ \Xhline{3\arrayrulewidth}




\multicolumn{7}{|c|}{autos} \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
\textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \hline
\multirow{3}{*}{\textbf{Time $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{1.11±0.112}     & \textbf{1.113±0.152}     & \textbf{1.111±0.115}    & \textbf{1.11±0.174}     & \textbf{1.227±0.139}   \\ \hline
              & \textbf{SVR}       & 9.416±0.371    & 9.389±0.285     & 9.124±0.354    & 9.468±0.568    & 9.576±0.456    \\ \hline
              & \textbf{Nu-SVR}    & 8.464±0.559    & 8.401±0.45      & 8.276±0.765    & 8.438±0.589    & 8.564±0.549    \\ \Xhline{3\arrayrulewidth}


\multirow{3}{*}{\textbf{$R^2$ $(\uparrow)$ }} 
              & \textbf{GBSVR}     & \textbf{0.872±0.037}    & \textbf{0.873±0.039}     & \textbf{0.872±0.025}    & \textbf{0.89±0.024}     & \textbf{0.875±0.028}    \\ \hline
              & \textbf{SVR}       & 0.74±0.068     & 0.725±0.093     & 0.701±0.087    & 0.789±0.068    & 0.715±0.137    \\ \hline
              & \textbf{Nu-SVR}    & 0.839±0.035    & 0.845±0.033     & 0.829±0.047    & 0.824±0.05     & 0.835±0.052    \\ \Xhline{3\arrayrulewidth}
              
\multirow{3}{*}{\textbf{MAE $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.265±0.032}    & \textbf{0.264±0.017}     & \textbf{0.266±0.034}    & \textbf{0.253±0.026}    & \textbf{0.262±0.021}    \\ \hline
              & \textbf{SVR}       & 0.356±0.033    & 0.353±0.033     & 0.367±0.035    & 0.322±0.034    & 0.355±0.056    \\ \hline
              & \textbf{Nu-SVR}    & 0.285±0.039    & 0.286±0.046     & 0.292±0.042    & 0.301±0.041    & 0.284±0.046    \\ \Xhline{3\arrayrulewidth}

\multirow{3}{*}{\textbf{MSE $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.119±0.022}    & \textbf{0.116±0.015}     & \textbf{0.121±0.024}    & \textbf{0.104±0.02}    & \textbf{0.116±0.014}    \\ \hline
              & \textbf{SVR}       & 0.249±0.071    & 0.256±0.078     & 0.275±0.06     & 0.192±0.032    & 0.26±0.106     \\ \hline
              & \textbf{Nu-SVR}    & 0.157±0.051    & 0.152±0.054     & 0.161±0.044    & 0.167±0.051    & 0.163±0.074    \\ \Xhline{3\arrayrulewidth}
\multirow{3}{*}{\textbf{RMSE $(\downarrow)$}} 
              & \textbf{GBSVR}     & \textbf{0.344±0.032}    & \textbf{0.339±0.023}     & \textbf{0.347±0.036}    & \textbf{0.321±0.031}    & \textbf{0.341±0.021}    \\ \hline
              & \textbf{SVR}       & 0.493±0.076    & 0.5±0.079       & 0.521±0.059    & 0.436±0.037    & 0.499±0.103    \\ \hline
              & \textbf{Nu-SVR}    & 0.391±0.065    & 0.384±0.068     & 0.397±0.056    & 0.404±0.064    & 0.394±0.086    \\ \Xhline{3\arrayrulewidth}





\multicolumn{7}{|c|}{machine} \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
\textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \hline
\multirow{3}{*}{\textbf{Time($\downarrow$)}} 
              & \textbf{GBSVR}  & \textbf{1.888±0.115}     & \textbf{1.902±0.136}     & \textbf{1.918±0.126}     & \textbf{1.993±0.177}    & \textbf{2.069±0.153}    \\ \hline
              & \textbf{SVR}    & 17.078±0.233    & 16.954±0.226    & 16.993±0.262    & 17.053±0.229   & 16.952±0.251   \\ \hline
              & \textbf{Nu-SVR} & 17.222±0.269    & 17.12±0.297     & 17.165±0.261    & 17.2±0.248     & 17.13±0.301    \\ 

\Xhline{3\arrayrulewidth}  


              
\multirow{3}{*}{\textbf{$R^2$($\uparrow$)}} 
              & \textbf{GBSVR}  & \textbf{0.836±0.021}     & \textbf{0.834±0.027}     & \textbf{0.835±0.032}     & \textbf{0.82±0.042}    & \textbf{0.826±0.036}    \\ \hline
              & \textbf{SVR}    & 0.744±0.065     & 0.743±0.053     & 0.718±0.103     & 0.734±0.057   & 0.746±0.046   \\ \hline
              & \textbf{Nu-SVR} & 0.746±0.035     & 0.748±0.036     & 0.753±0.037     & 0.749±0.036   & 0.747±0.034   \\ 

\Xhline{3\arrayrulewidth} 
              
\multirow{3}{*}{\textbf{MAE  $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.311±0.023}     & \textbf{0.311±0.03}     & \textbf{0.308±0.023}     & \textbf{0.321±0.023}    & \textbf{0.32±0.021}    \\ \hline
              & \textbf{SVR}    & 0.376±0.071     & 0.384±0.068    & 0.388±0.078     & 0.385±0.069   & 0.379±0.062   \\ \hline
              & \textbf{Nu-SVR} & 0.392±0.033     & 0.392±0.033    & 0.39±0.037      & 0.392±0.036   & 0.389±0.036   \\ 

\Xhline{3\arrayrulewidth}


\multirow{3}{*}{\textbf{MSE  $(\downarrow)$}} 
               & \textbf{GBSVR}  & \textbf{0.161±0.026}     & \textbf{0.161±0.025}     & \textbf{0.16±0.027}     & \textbf{0.173±0.022}    & \textbf{0.168±0.026}    \\ \hline
              & \textbf{SVR}    & 0.258±0.104     & 0.257±0.088    & 0.288±0.155     & 0.267±0.094   & 0.252±0.074   \\ \hline
              & \textbf{Nu-SVR} & 0.247±0.031     & 0.245±0.029    & 0.241±0.036     & 0.244±0.033   & 0.247±0.034   \\ 

\Xhline{3\arrayrulewidth} 


\multirow{3}{*}{\textbf{RMSE  $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.4±0.033}       & \textbf{0.401±0.031}     & \textbf{0.399±0.033}     & \textbf{0.414±0.027}    & \textbf{0.409±0.031}    \\ \hline
              & \textbf{SVR}    & 0.499±0.091     & 0.501±0.079     & 0.522±0.126     & 0.51±0.082     & 0.498±0.067    \\ \hline
              & \textbf{Nu-SVR} & 0.496±0.031     & 0.494±0.03      & 0.489±0.036     & 0.493±0.033    & 0.495±0.033    \\ 

\Xhline{3\arrayrulewidth}  



\multicolumn{7}{|c|}{Real Estate Valuation} \\ \Xhline{3\arrayrulewidth}
\multicolumn{2}{|c|}{} & \multicolumn{5}{|c|}{\textbf{Noise Percentage}} \\ \Xhline{3\arrayrulewidth}
\textbf{Metric}     & \textbf{Methods}       & 0              & \multicolumn{1}{c|}{0.05}         & 0.1            & 0.15           & 0.2            \\ \hline
\multirow{3}{*}{\textbf{Time $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{7.335±1.151}     & \textbf{7.121±0.633}     & \textbf{6.86±0.881}      & \textbf{8.004±1.186}    & \textbf{7.522±0.642}    \\ \hline
              & \textbf{SVR}    & 95.774±0.917    & 94.793±0.865    & 94.927±0.703    & 96.663±1.722   & 95.103±0.671   \\ \hline
              & \textbf{Nu-SVR} & 93.068±1.192    & 92.017±1.501    & 91.805±0.768    & 94.193±1.282   & 91.832±0.746   \\ 

\Xhline{3\arrayrulewidth}  


              
\multirow{3}{*}{\textbf{$R^2$ $(\uparrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.63±0.075 }     & \textbf{0.629±0.069}     & \textbf{0.633±0.077}     & \textbf{0.637±0.073}    & \textbf{0.625±0.071}    \\ \hline
              & \textbf{SVR}    & 0.542±0.059     & 0.546±0.07      & 0.535±0.062     & 0.555±0.066    & 0.531±0.057    \\ \hline
              & \textbf{Nu-SVR} & 0.548±0.061     & 0.557±0.071     & 0.54±0.065      & 0.553±0.059    & 0.53±0.06      \\ 

\Xhline{3\arrayrulewidth}  


              
\multirow{3}{*}{\textbf{MAE $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.403±0.034}     & \textbf{0.4±0.032}       & \textbf{0.4±0.033}       & \textbf{0.395±0.032}    & \textbf{0.403±0.03}     \\ \hline
              & \textbf{SVR}    & 0.503±0.035     & 0.5±0.037       & 0.507±0.035     & 0.499±0.039    & 0.508±0.03     \\ \hline
              & \textbf{Nu-SVR} & 0.5±0.034       & 0.495±0.04      & 0.504±0.038     & 0.498±0.03     & 0.511±0.036    \\ 

\Xhline{3\arrayrulewidth}  



\multirow{3}{*}{\textbf{MSE $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.374±0.132}     & \textbf{0.375±0.126}     & \textbf{0.372±0.134}     & \textbf{0.367±0.127}    & \textbf{0.379±0.128}    \\ \hline
              & \textbf{SVR}    & 0.455±0.098     & 0.45±0.1        & 0.463±0.105     & 0.443±0.105    & 0.466±0.104    \\ \hline
              & \textbf{Nu-SVR} & 0.448±0.098     & 0.439±0.103     & 0.458±0.107     & 0.444±0.096    & 0.467±0.101    \\ 

\Xhline{3\arrayrulewidth} 


\multirow{3}{*}{\textbf{RMSE  $(\downarrow)$}} 
              & \textbf{GBSVR}  & \textbf{0.604±0.099}     & \textbf{0.605±0.094}     & \textbf{0.601±0.1}       & \textbf{0.598±0.096}    & \textbf{0.608±0.096}    \\ \hline
              & \textbf{SVR}    & 0.671±0.069     & 0.667±0.071     & 0.676±0.073     & 0.661±0.075    & 0.679±0.072    \\ \hline
              & \textbf{Nu-SVR} & 0.666±0.069     & 0.659±0.075     & 0.672±0.075     & 0.663±0.069    & 0.68±0.07      \\ 

\Xhline{3\arrayrulewidth}  



\end{tabular}
\label{result_table1}
\end{table*}



